Algorithmic Analysis of Qualitative and Quantitative Termination Problems for Affine Probabilistic Programs

In this paper, we consider termination of probabilistic programs with real-valued variables. The questions concerned are: 1. qualitative ones that ask (i) whether the program terminates with probability 1 (almost-sure termination) and (ii) whether the expected termination time is finite (finite termination); 2. quantitative ones that ask (i) to approximate the expected termination time (expectation problem) and (ii) to compute a bound B such that the probability to terminate after B steps decreases exponentially (concentration problem). To solve these questions, we utilize the notion of ranking supermartingales which is a powerful approach for proving termination of probabilistic programs. In detail, we focus on algorithmic synthesis of linear ranking-supermartingales over affine probabilistic programs (APP's) with both angelic and demonic non-determinism. An important subclass of APP's is LRAPP which is defined as the class of all APP's over which a linear ranking-supermartingale exists. Our main contributions are as follows. Firstly, we show that the membership problem of LRAPP (i) can be decided in polynomial time for APP's with at most demonic non-determinism, and (ii) is NP-hard and in PSPACE for APP's with angelic non-determinism; moreover, the NP-hardness result holds already for APP's without probability and demonic non-determinism. Secondly, we show that the concentration problem over LRAPP can be solved in the same complexity as for the membership problem of LRAPP. Finally, we show that the expectation problem over LRAPP can be solved in 2EXPTIME and is PSPACE-hard even for APP's without probability and non-determinism (i.e., deterministic programs). Our experimental results demonstrate the effectiveness of our approach to answer the qualitative and quantitative questions over APP's with at most demonic non-determinism.

==> quan-preamble.tex <==

\section{\LRAPP s: Quantitative Analysis}
In this section we consider the quantiative questions for \LRAPP s.
We start with an example to show that there exist programs $P$ 
in \LRAPP s such that both the expected termination time $\Eval(P)$, 
and the probability $\Thr(P,x)$ to terminate after a given number 
$x$ of steps are {\em irrational.}

\newsavebox{\figexampleirrational}
\begin{lrbox}{\figexampleirrational}
\begin{lstlisting}[mathescape]
x:=1;
while $x\le 10$ do $x:=x+5+\mathrm{exp}(1)$ od
\end{lstlisting}
\end{lrbox}
\begin{figure}[h]
\centering
\usebox{\figexampleirrational}
\caption{An example where values can be irrational}
\label{fig:irrational}
\end{figure}

\begin{example}
Consider the example in Fig.~\ref{fig:irrational} where $\mathrm{exp}(1)$ represents a random variable that 
observes the negative exponential distribution with rate $1$.
Then one can verify that $\probm(T>1)=1-e^{-4}$ and 
$\expv(T)=1\cdot e^{-4}+2\cdot (1-e^{-4})=2-e^{-4}$, both of them being irrational since $e$ is a transcendental number.   
\end{example}


While the above example is for continuous distribution, if we 
restrict to programs $P$ with discrete distributions and rational probabilities,
then $\Thr(P,x)$ is rational, because we can compute the termination
probability in a finite stochastic game for $x$ steps.
However, the following example shows that even for discrete probabilistic
choices, $\Eval(P)$ can be irrational.

{\bf KRISH: EXAMPLE FROM PETR.}

Given that the expected terimnation time or the termination probability for given
number of steps can be irrational, instead of computing them exactly we consider
computational aspects of \emph{approximating} these values, with respect to additive 
or relative error. 
We also consider the problem of computing concentraion bounds.
Our main results are summarized below (note for the approximation problems we write
$\PSPACE$-hardness that the corresponding decision problem is hard; 
see Lemma~\ref{}).


\begin{theorem}\label{thm:quan_lrapp}
The following assertions hold for programs in \LRAPP.
\begin{compactenum}

\item Approximating $\Eval(P)$ (resp., $\Thr(P,x)$, for $x \in \Nat_{\geq 0}$)
is $\PSPACE$-hard, even for deterministic programs $P$ without probabilities 
in \LRAPP.

\item A concentration bound $B$ can be computed in the same complexity as for 
qualitative analysis (i.e., in polynomial time with only demonic non-determinism,
and in $\PSPACE$ in the general case). 
Moreover, the bound $B$ is atmost exponential.
\end{compactenum}
\end{theorem}


\smallskip\noindent{\em Significance of our concentration result.}
First, note that the bound $B$ is exponential, and our result (Lemma~\ref{})
shows that there exists deterministic programs in \LRAPP\ that terminates
exactly after exponential number of steps (i.e., an exponential bound for
$B$ is asymptotically optimal for \LRAPP s.
Second, our concentration result imply decidability of the approximation 
problems.
Let $C$ be a concentration bound and $\epsilon>0$ be an approximation parameter. 
Let $C'= O(C/\epsilon)$.
We discuss the approximation for the expectation problem.
The approximation solution is as follows:
(1)~compute $\epsilon/(2C')$ approximation of the continuous distribution; 
(2)~unfold the program upto $C'$ steps, and explicitly compute an $\epsilon/2$-approximation
$e$ of the expected termination within $C'$ steps.
Then $e$ is an $\epsilon$-approximation for $\Eval(P)$. 
Note that the computation for $C'$ steps can be exponential in $C'$ (as the 
program may contain statements of the form $x:= 1/2 x$).
The computation for probabilistic problem is similar. 
Since we establish an exponential bound $B$ for concentration, we obtain a
$\TWOEXPTIME$ result for approximation.



\begin{corollary}
Approximating $\Eval(P)$ (resp., $\Thr(P,x)$, for $x \in \Nat_{\geq 0}$)
for programs $P$ in \LRAPP\ can be done in $\TWOEXPTIME$.
\end{corollary}

In the next subsection we establish the first item of Theorem~\ref{thm:quan_lrapp},
and the second item in the following subsection.


